Maximum Weight Convex Polytope

We study the maximum weight convex polytope problem, in which the goal is to find a convex polytope maximizing the total weight of enclosed points. Prior to this work, the only known result for this problem was an $O(n^3)$ algorithm for the case of $2$ dimensions due to Bautista et al. We show that the problem becomes $\mathcal{NP}$-hard to solve exactly in $3$ dimensions, and $\mathcal{NP}$-hard to approximate within $n^{1/2-\epsilon}$ for any $\epsilon > 0$ in $4$ or more dimensions. %\polyAPX-complete in $4$ dimensions even with binary weights. We also give a new algorithm for $2$ dimensions, albeit with the same $O(n^3)$ running time complexity as that of the algorithm of Bautsita et al.

==> styles/custom.tex <==

% -------------------------------------------------------
%  Custom Definitions
% -------------------------------------------------------


\newcommand{\OPT}{\ensuremath{\mathop{\mathrm{OPT}}}}
\newcommand{\APX}{\ensuremath{\mathop{\mathrm{APX}}}}
\newcommand{\ALG}{\ensuremath{\mathop{\mathrm{ALG}}}}


